Autobidders with Budget and ROI Constraints: Efficiency, Regret, and Pacing Dynamics

We study a game between autobidding algorithms that compete in an online advertising platform. Each autobidder is tasked with maximizing its advertiser's total value over multiple rounds of a repeated auction, subject to budget and return-on-investment constraints. We propose a gradient-based learning algorithm that is guaranteed to satisfy all constraints and achieves vanishing individual regret. Our algorithm uses only bandit feedback and can be used with the first- or second-price auction, as well as with any "intermediate" auction format. Our main result is that when these autobidders play against each other, the resulting expected liquid welfare over all rounds is at least half of the expected optimal liquid welfare achieved by any allocation. This holds whether or not the bidding dynamics converges to an equilibrium.

==> expt-plots.tex <==

\begin{figure}[!b]
\centering
\includegraphics[width=0.99\textwidth]{{\FigPath}mu_convergence_T=9001.pdf}
\captionsetup{justification=centering}
\caption{Multiplier dynamics for $\mu_{1,t}$, as a function of time $t$.\\
The plots show that the trajectory of $\mu_{1,t}$ is very stable across runs (else, there would have been a noticeable shaded area), and \textbf{that non-convergence is \emph{a} typical outcome.}}
\label{fig:mu}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.99\textwidth]{{\FigPath}budget_violation_T=9001.pdf}
\captionsetup{justification=centering}
\caption{Budget Slackness \eqref{eq:slack-expts}: empirical CDF  over all agents and all runs.\\
Both our algorithm and BOMW \citep{feng2022online} do not violate the budget constraint.}
\label{fig:budget_1}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.99\textwidth]{{\FigPath}budget_violation_2_T=9001.pdf}
\captionsetup{justification=centering}
\caption{Budget Slackness \eqref{eq:slack-expts}: empirical CDF  over all agents and all runs.\\ The naive baselines exhibit large constraint violations.}
\label{fig:budget_2}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.99\textwidth]{{\FigPath}roi_violation_T=9001.pdf}
\captionsetup{justification=centering}
\caption{ROI Slackness \eqref{eq:slack-expts}: empirical CDF  over all agents and all runs. \\
Our algorithm does not violate the ROI constraint, while BOMW's violations are very small.}
\label{fig:roi_1}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=\textwidth]{{\FigPath}roi_violation_2_T=9001.pdf}
\captionsetup{justification=centering}
\caption{ROI Slackness \eqref{eq:slack-expts}: empirical CDF  over all agents and all runs.\\ The naive baselines exhibit large constraint violations.}
\label{fig:roi_2}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.99\textwidth]{{\FigPath}liquid_welfare_T=9001.pdf}
\captionsetup{justification=centering} % Centering the caption
\caption{Time-averaged liquid welfare $\overline{\LW}_t$ as a function of time $t$. \\All implemented algorithms enjoy similar liquid welfare value.}
\label{fig:liquid_welfare}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=0.99\textwidth]{{\FigPath}regret_T=9001.pdf}
\captionsetup{justification=centering}
\caption{The time-averaged static regret for agent $1$,
    $\bar{R}(t) = \frac{1}{t}\, \mathtt{StaticReg}_1(t)$,
vs time $t$.
\\ $\bar{R}(t)$ is averaged over runs, with shaded area indicating the (small) discrepancy between the runs.
\\
$\bar{R}(t)$ substantially decreases over time and appears to tend to $0$, for both algorithms. \\ BOMW performs somewhat better, as far as $\bar{R}(t)$ is concerned.}
\label{fig:individual_regret_normal}
\end{figure}

\begin{figure}[!t]
%\centering
\hspace{-15mm}\includegraphics[width=1.2\textwidth]{{\FigPath}regret_loglog_T=9001.pdf}
\captionsetup{justification=centering}
\caption{Static regret for agent $1$,
    $R(t) = \mathtt{StaticReg}_1(t)$,
as a function of $t$. \\ The plot is presented in log-log axes, namely $\log\rbr{\max\rbr{R(t),0}}$ vs $\log(t)$.\\
10 out of 12 plots are near-straight lines, indicating a good fit to $R(T) = T^{\RegPow}$ for some $\RegPow\in(0,1)$.}
%Individual regret in log-log axis. $x$ ($y$)-axis corresponds to the logarithmic value of the horizon (averaged regret clipped by $0$).
%The fitted curve has slope ranging from $[-1.2, -0.3]$, showing that our algorithm empirically enjoys sublinear standard regret.}
\label{fig:individual_regret}
\end{figure}

